The Formalization of two Computational Models in Dafny

We describe the formalization in Dafny of two computational models, Turing Machines and the Lambda Calculus. We present several application of the formalizations: machine proofs of termination for Turing machines, Dafny proofs for Church encodings, and a mechanized proof of the Church-Rosser theorem.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.6}{10.4204/EPTCS.452.6}}

